Controllable Text Generation in the Instruction-Tuning Era

While most research on controllable text generation has focused on steering base Language Models, the emerging instruction-tuning and prompting paradigm offers an alternate approach to controllability. We compile and release ConGenBench, a testbed of 17 different controllable generation tasks, using a subset of it to benchmark the performance of 9 different baselines and methods on Instruction-tuned Language Models. To our surprise, we find that prompting-based approaches outperform controllable text generation methods on most datasets and tasks, highlighting a need for research on controllable text generation with Instruction-tuned Language Models in specific. Prompt-based approaches match human performance on most stylistic tasks while lagging on structural tasks, foregrounding a need to study more varied constraints and more challenging stylistic tasks. To facilitate such research, we provide an algorithm that uses only a task dataset and a Large Language Model with in-context capabilities to automatically generate a constraint dataset. This method eliminates the fields dependence on pre-curated constraint datasets, hence vastly expanding the range of constraints that can be studied in the future.

==> figures/excitement_examples.tex <==
\begin{figure*}
\begin{Verbatim}[commandchars=\\\{\}, fontsize=\small,frame=single]
\textcolor{red}{Difficult Prompt}: 

\textbf{Greedy}: 

\textbf{Reranking}: 

\textbf{ZeroShot}: 

\textbf{FewShot}: 

\textbf{Human}: 

\textbf{FUDGE}: 

\textbf{NeuroLogic}:

\textbf{DEXPERTS}:

\textbf{Air}: 

\textcolor{cyan}{Easy Prompt}: 

\textbf{Greedy}: 

\textbf{Reranking}: 

\textbf{ZeroShot}: 

\textbf{FewShot}: 

\textbf{Human}: 

\textbf{FUDGE}: 

\textbf{NeuroLogic}:

\textbf{DEXPERTS}: 

\textbf{Air}: 
\end{Verbatim}
    \caption{Randomly selected examples from the Exciting Continuation task after partitioning results using the average excitement score as determined by human annotation.}    
    \label{fig:excitement-example}
\end{figure*}

==> figures/sensationalism_examples.tex <==
\begin{figure*}
\begin{Verbatim}[commandchars=\\\{\}, fontsize=\small,frame=single]
\textcolor{red}{Difficult Prompt}: 

\textbf{Greedy}: 

\textbf{Reranking}: 

\textbf{ZeroShot}: 

\textbf{FewShot}: 

\textbf{Human}: 

\textbf{FUDGE}: 

\textbf{NeuroLogic}:

\textbf{DEXPERTS}:

\textbf{Air}: 

\textcolor{cyan}{Easy Prompt}: 

\textbf{Greedy}: 

\textbf{Reranking}: 

\textbf{ZeroShot}: 

\textbf{FewShot}: 

\textbf{Human}: 

\textbf{FUDGE}: 

\textbf{NeuroLogic}:

\textbf{DEXPERTS}: 

\textbf{Air}: 
\end{Verbatim}
    \caption{Randomly selected examples from the Sensationalistic Continuation task after partitioning results using the average sensationalism score as determined by human annotation.}    
    \label{fig:sensationalism-example}
\end{figure*}

==> figures/topic_examples.tex <==
\begin{figure*}
\begin{Verbatim}[commandchars=\\\{\}, fontsize=\small,frame=single]
\textcolor{red}{Difficult Prompt}: 

\textbf{Greedy}: 

\textbf{Reranking}: 

\textbf{ZeroShot}: 

\textbf{FewShot}: 

\textbf{Human}: 

\textbf{FUDGE}: 

\textbf{NeuroLogic}:

\textbf{DEXPERTS}:

\textbf{Air}: 

\textcolor{cyan}{Easy Prompt}: 

\textbf{Greedy}: 

\textbf{Reranking}: 

\textbf{ZeroShot}: 

\textbf{FewShot}: 

\textbf{Human}: 

\textbf{FUDGE}: 

\textbf{NeuroLogic}:

\textbf{DEXPERTS}: 

\textbf{Air}: 
\end{Verbatim}
    \caption{Randomly selected examples from the Topic Control task after partitioning results using the average topic compliance score as determined by human annotation.}    
    \label{fig:topic-example}
\end{figure*}
